Deepfake Text Detection: Limitations and Opportunities

Recent advances in generative models for language have enabled the creation of convincing synthetic text or deepfake text. Prior work has demonstrated the potential for misuse of deepfake text to mislead content consumers. Therefore, deepfake text detection, the task of discriminating between human and machine-generated text, is becoming increasingly critical. Several defenses have been proposed for deepfake text detection. However, we lack a thorough understanding of their real-world applicability. In this paper, we collect deepfake text from 4 online services powered by Transformer-based tools to evaluate the generalization ability of the defenses on content in the wild. We develop several low-cost adversarial attacks, and investigate the robustness of existing defenses against an adaptive attacker. We find that many defenses show significant degradation in performance under our evaluation scenarios compared to their original claimed performance. Our evaluation shows that tapping into the semantic information in the text content is a promising approach for improving the robustness and generalization performance of deepfake text detection schemes.

==> responses.tex <==
\clearpage
\section{Summary of Changes}

\noindent We thank the reviewers for their insightful feedback. In Section~\ref{sec:mjrev}, we start by describing how we addressed the recommended changes for the major revision. Later, we respond to comments made by individual reviewers in Sections~\ref{sec:reva},~\ref{sec:revb},~\ref{sec:revc}, and~\ref{sec:revd}.

We have incorporated all the feedback we received. We believe this revision has improved our work. This includes efforts to improve writing, while also providing enough details to help the reader understand our methodologies and key takeaways. Empirical work with large language models requires significant computational effort. For example, certain small configuration changes, such as changing the context window of a LM, can trigger significant additional computational effort to update the results. To incorporate all the feedback, this revision work required us to redefine certain evaluation settings, regenerate tens of thousands of text samples and rerun hundreds of evaluation experiments. All these changes resulted in approximately 112 hours of data generation efforts and around 1,083 hours of GPU computation time. 
% and 458 experiments to rerun.


\subsection{Recommended Changes for Major Revision}
\label{sec:mjrev}
\noindent \textbf{Major-Rev, Comment-1.} \texttt{``improve discussion of related work with pointers included in reviews''}

\textit{Response: } 
This is regarding Reviewer D's suggestion to add a discussion on the similarity/difference between our work and existing work on the robustness of deepfake image detection.
To address this, we added a discussion titled ``Deepfake text detection Vs. deepfake image detection.'' in Section~\ref{sec:discussion}. The discussion is replicated below: \\
\textit{Deepfake text detection Vs. deepfake image detection.} Deepfake image detection and deepfake text detection both aim to detect synthetic content generated by deep generative models. That said, these two fields hardly share the same set of technical methodologies in generating and detecting synthetic content due to the discrete nature of text. Similar to the text domain, researchers have also demonstrated impressive performance in detecting deepfake images~\cite{frank2020leveraging, wang2020cnn} This has prompted work investigating the adversarial robustness of deepfake image detectors~\cite{carlini2020evading, gandhi2020adversarial, cao2021understanding}. In a similar way, our work is the first to systematically explore real-world performance and adversarial robustness of deepfake text detectors. While the image domain has primarily focused on adversarial perturbations, our work also explores low-cost evasion strategies that change the content generation process. Note that the adversarial attacks studied for the image domain are not directly applicable to the text domain. If we compare detection schemes in the two domains, more progress has been made on understanding the use of semantic features for deepfake image detection~\cite{li2018ictu, li2018exposing, ciftci2020fakecatcher, matern2019exploiting}. An example is a method that looks for eye blinking artifacts~\cite{jung2020deepvision} to detect deepfake images. However, in the text domain, \fast{} is the only approach that leverages semantic features (entity-based), and there is scope for more work to be done in this direction.

 
% \textit{Response: } 
% This is regarding RevD, Comment-1 in Section~\ref{sec:revd}, which suggests to add a discussion on the similarity/difference between our work and existing work on the robustness of deepfake image/video detection.

% To address this, we made the following change: (1) We added a discussion section titled \textbf{``Deepfake text detection VS. deepfake image/video detection.''} in Section~\ref{sec:discussion} regarding the relevance between our work and existing work in deepfake image/video detection.

% For your reading convenience, here is the detailed discussion: Deepfake image/video detection and deepfake text detection both aim to detect synthetic content generated by generative models. 
% This work shares the same motivation as existing work that focuses on the robustness of deepfake image/video detection~\cite{carlini2020evading, gandhi2020adversarial, cao2021understanding}. 
% In the image/video domain, attackers are able to craft different types of adversarial attacks to evade detection, including adding adversarial perturbations, backdoor attacks, etc.
% Similarly, our work also explored a range of adversarial attacks for evading deepfake text detection.
% That said, these two fields hardly share the same set of technical methodologies. Due to the discrete nature of text,
% adversarial attacks discussed for deepfake image/video detectors are not directly applicable to deepfake text detectors, and vice versa. In other words, low-cost attacks proposed in our work 
% are entirely novel techniques.
%  In the image/video domain, there are plenty of existing work which identifies abnormal semantic features such as abnormal eye blinking in the synthetic content.~\cite{li2018ictu, li2018exposing}.
%  However, there is less work in the text domain which employs semantic features for detecting deepfake text. 
%  We believe our discussion on adversarial robustness can pave the way for future advanced defenses to a great extent. 
 






\noindent \textbf{Major-Rev, Comment-2.} \texttt{``improve writing and clarify experimental details and choices''}

\textit{Response: } As this is an overarching comment, we provide detailed responses to individual comments by reviewers in later sections of this document. We have revised all the sections in the paper with a focus on improving clarity. We have ensured that details of all our experiments are available for the reader to understand our methodology. We also added/updated additional sections in the Appendix, including Sections~\ref{gruen_subscores},~\ref{sec:wild_text_quality},~\ref{sec:other_defenses},~\ref{sec:gltr_grid_search},~\ref{sec:exp_details} and~\ref{sec:dft_details} providing more experimental details.

% This comment is based on the following 4 points raised by individual reviewers: 

% (1) Reviewer C pointed out that the finding ``\textit{Robustly pre-trained bidirectional models generalize better than unidirectional models}'' (Finding 2 in the current draft) is not convincing.  We addressed this concern under RevC, Comment-6 in Section~\ref{sec:revc}.

% (2) Reviewer D pointed out that explanation of the finding ``\textit{Defenses trained on conditionally generated text are not able to detect unconditionally generated text}'' (Finding 6 in the current draft) is not clear. We addressed this concern under RevD, Comment-3 in Section~\ref{sec:revd}

% (3) Review D pointed out that the explanation of the finding ``\textit{\ourattack{} can generate transferable adversarial samples}'' (Finding 7 in the current draft) is not convincing.  We addressed this concern under RevD, Comment-2 in Section~\ref{sec:revd}.

% (4) To improve experimental details and choices, we added Section~\ref{sec:exp_details} in Appendix to present all the experimental details and choices.

% (1) Reviewer C pointed out that the finding ``\textit{Robustly pre-trained bidirectional models generalize better than unidirectional models}'' (Finding 2 in the current draft) is not convincing.  We addressed this concern under RevC, Comment-6 in Section~\ref{sec:revc}.

% (2) Reviewer D pointed out that explanation of the finding ``\textit{Defenses trained on conditionally generated text are not able to detect unconditionally generated text}'' (Finding 6 in the current draft) is not clear. We addressed this concern under RevD, Comment-3 in Section~\ref{sec:revd}

% (3) Review D pointed out that the explanation of the finding ``\textit{\ourattack{} can generate transferable adversarial samples}'' (Finding 7 in the current draft) is not convincing.  We addressed this concern under RevD, Comment-2 in Section~\ref{sec:revd}.

% (4) To improve experimental details and choices, we added Section~\ref{sec:exp_details} in Appendix to present all the experimental details and choices.



% To address this, we made the following changes: (1) We addressed all the clarity concerns raised by each reviewer in the main body text. Particularly, We better explain Finding 3 and Finding 8, and Finding 10 to clarify concerns raised by Review C- Quote 6, Review D - Quote 3 and Review D - Quote 2, respectively. (2) We improve the clarity of DFTFooler by adding detailed technical steps in Section~\ref{sec:adaptive-attack-methods}, illustration (Figure~\ref{fig:dftfooler}) and pseudo algorithm (Algorithm~\ref{alg: dftfooler-algo}). 
% (3) We additionally added Section~\ref{sec:exp_details} in Appendix to present all the experimental details and choices.  

\begin{figure}[!t]
\centering
\includegraphics[width=0.9\columnwidth]{figs/dist_bar.pdf}
%\vspace{-2ex}
\caption{The distribution distance between the training set and the test sets (including baseline test set and \textit{In-the-wild} test sets) of \gbert{} and \grover{}.}
%\vspace{-4ex}
\label{fig:dist_bar_response}
\end{figure}


\noindent \textbf{Major-Rev, Comment-3.} \texttt{``interpret the results with a metric to measure the distance between the two distributions''}

\textit{Response: } 
This is regarding Reviewer A's suggestion to analyze the distribution shift between the training set of the detector and the In-the-wild set, so that the percentage change in F1-score $\Delta F1$ can be interpreted relative to it. 

To address this concern, we conducted experiments to interpret the correlation between the distribution shift and the performance change. In a nutshell, we observe an obvious performance drop when there is a significant distribution shift between the training distribution and testing distribution. On the other hand, we observe a performance boost when the training distribution and testing distribution are closer. We added this analysis in Section~\ref{sec:detection_performance_defenses} of the paper.

%Detailed experiment results are presented in Figure~\ref{fig:dist_bar_response} below. 

We replicate the details here: Open-domain defenses show significant degradation in performance when applied to synthetic text in the wild, while defenses trained on data from a specific domain are able to detect In-the-wild data from that domain. We further investigate the performance differences between the open-domain and the news domain defenses. Our hypothesis is that this can be attributed to distribution shift or distributional differences between data in the wild and the original datasets used to train/evaluate the defenses. To study this, we choose \gbert{} from the open-domain category, and \grover{} from the news category. We use a simple metric, average-linkage~\cite{moseley2017approximation}, to measure the distribution distance between two synthetic datasets. Given two synthetic datasets, $X$, and $Y$, we define the distribution distance as $D(X,Y)$. To represent a dataset's distribution, we randomly select 1,000 articles (or all available samples if there are fewer samples) from the dataset, and then extract the hidden state of the special [CLS] token (used as the input to the classifier) in each article from the detector as its representation. Thus $X$ and $Y$ each includes 1000 embedding vectors. Larger values of $D(X, Y)$ indicate a larger distribution shift.

For each defense, we compute 2 types of distance measures: (1) Distance $D(X_{train}, Y_{test})$ between its training dataset $X_{train}$ and its original test set $Y_{test}$ (\ie test set used in Table~\ref{tab:defenses-setup}). (2) Distance $D(X_{train}, Y_{wild})$ between its training dataset and each of the In-the-wild datasets $Y_{wild}$.
We expect that $D(X_{train}, Y_{wild})$ is greater than $D(X_{train}, Y_{test})$ if the defense's performances on \textit{In-the-wild} datasets degrade, and $D(X_{train}, Y_{wild})$ is closer to $D(X_{train},Y_{test})$ if the detection performances are similar. 
Results are in Figure~\ref{fig:dist_bar_response}. All the $D(X_{train},Y_{wild})$ are significantly greater than $D(X_{train},Y_{test})$ for \gbert{}, but not for \grover{}. This observation is in line with our hypothesis.

% \textit{Response: } \jiameng{synced with main body text}
% This is regarding RevA, Comment-3 in Section~\ref{sec:reva}, which suggests analyzing the distribution shift between the training set of the detector and the In-the-wild set so that the percentage change in F1-score $\Delta F1$ can be interpreted relative to it. 

% To address this concern, we conducted experiments to interpret the correlation between the distribution shift and the performance change. In a nutshell, we observe an obvious performance drop when there is a significant distribution shift between the training distribution and testing distribution. On the other hand, we observe a performance boost when the training distribution and testing distribution are closer. Detailed experiment results are presented in Figure~\ref{fig:dist_bar_response} below. 

% For your reading convenience, here is how we addressed this: We further investigate the performance differences between the open-domain and the news domain defenses. Our hypothesis is that this can be attributed to distribution shift or distributional differences between data in the wild and the original datasets used to train/evaluate the defenses. To study this, we choose \gbert{} from the open-domain category, and \grover{} from the news category. We use a simple metric, average-linkage~\cite{moseley2017approximation}, to measure the distribution distance between two synthetic datasets. Given two synthetic datasets, $X$, and $Y$, we define the distribution distance as $D(X,Y)$. To represent a dataset's distribution, we randomly select 1,000 articles (or all available samples if there are fewer samples) from the dataset, and then extract the hidden state of the special [CLS] token (used as the input to the classifier) in each article from the detector as its representation. Thus $X$ and $Y$ each includes 1000 embedding vectors. Larger values of $D(X, Y)$ indicate a larger distribution shift.

% For each defense, we compute 2 types of distance measures: (1) Distance $D(X_{train}, Y_{test})$ between its training dataset $X_{train}$ and its original test set $Y_{test}$ (\ie test set used in Table~\ref{tab:defenses-setup}). (2) Distance $D(X_{train}, Y_{wild})$ between its training dataset and each of the In-the-wild datasets $Y_{wild}$.
% We expect that $D(X_{train}, Y_{wild})$ is greater than $D(X_{train}, Y_{test})$ if the defense's performances on \textit{In-the-wild} datasets degrade, and $D(X_{train}, Y_{wild})$ is closer to $D(X_{train},Y_{test})$ if the detection performances are similar. 
% Results are in Figure~\ref{fig:dist_bar_response}. All the $D(X_{train},Y_{wild})$ are significantly greater than $D(X_{train},Y_{test})$ for \gbert{}, but not for \grover{}. This observation is in line with our hypothesis.



% For your reading convenience, here is how we addressed this: To better interpret the performance degradation, we analyze the distribution shift between training samples and in-the-wild samples. Specifically, we analyze \gbert{} which suffers serious performance degradation, and \grover{} that mostly maintains its original detection performance. 
% For each defense, we first measure the distribution distance between its training samples and its testing samples (based on which we obtain evaluation results in Table~\ref{tab:defenses-setup}), and we call this distance \textit{D-B}. We then measure the distribution distance between its training samples and in-the-wild samples (based on which we obtain evaluation results in Table~\ref{sec:in_the_wild_datasets}), and we call this distance D-W. To represent each dataset distribution, we firstly randomly select 1,000 text samples from each dataset, and then feed each text sample to the detector to extract the [CLS] hidden state embedding as its latent representation.~\footnote{In both \gbert{} and \grover{}, the [CLS] hidden state embedding is fed into the classification layer to predict the label.}
% We thus obtain 1,000 embedding vectors from each dataset distribution. To measure the distance between two dataset distribution, we compute the 
% Average-linkage~\footnote{Average-linkage is where the distance between each pair of observations in each cluster are added up and divided by the number of pairs to get an average inter-cluster distance.} between embedding vectors of two datasets, following Equation~\ref{eqn: average_linkage}, where $D(x_i, y_j)$ computes the cosine distance between vector $x$ and vector $y$~\footnote{\url{https://docs.scipy.org/doc/scipy/reference/generated/scipy.spatial.distance.cosine.html}}.
% Following the above strategy, we calculate \textit{D-B} and \textit{D-W} (for each available in-the-wild dataset) for \gbert{} and \grover{}, and present results in Table~\ref{tab:distribution_shift}. We observe that, for \gbert{} which suffers serious performance degradation, all the \textit{D-W} are larger than its \textit{D-B}. For \grover{},  the \textit{D-W} on AI-Writer is smaller than \grover{}'s \textit{D-B} because \grover{}'s detection  performance on AI-Writer increased by 0.6\%.



\noindent \textbf{Major-Rev, Comment-4.} \texttt{``Lack of sufficient technical details regarding process of adversarial examples generation''}

\textit{Response: } The reviewer is suggesting to add more technical details of our proposed adversarial attack \ourattack{}.
To address this, in Section~\ref{sec:dftfooler_tech_details}, we added more details of our \ourattack{} pipeline. We will also release the code for our \ourattack{} attack, once our work is published. We provide the technical details here again:

First, \ourattack{} scans a given article to choose the top $N$, most confidently predicted words according to the chosen LM, for replacement. 
The importance of a word is determined by the absolute rank of its token probability predicted by the LM.~\footnote{For words that are split into multiple sub-tokens, we use the probability prediction of the first sub-token in the word.} \ourattack{} does not perturb stop words. More details about using a LM to find important words are described in the Appendix~\ref{sec:dft_details}.

The second step is to find replacement words, while preserving semantics. To find a synonym for replacement, we use the methodology used by TextFooler~\cite{jin2020bert}, and adapt it to our setting to not require queries to the victim model. 
For a targeted word, there are 4 sub-steps to find a valid synonym: \textit{(1) Synonym Extraction:} We first extract a candidate set of synonyms for the targeted word as its possible word replacements. Synonym candidates are chosen according to the cosine similarity between the word embeddings of the targeted word and every other word in the vocabulary. We use word embeddings from~\cite{mrkvsic2016counter} which are specially curated for finding synonyms. \textit{(2) POS Checking}: The goal of POS checking is to assure that the grammar of the perturbed text remains the same. We will only keep synonyms with the same part-of-speech (POS) tag as the targeted word.
\textit{(3) Semantic Similarity Checking:} This step ensures that the sentence semantics before and after replacing the targeted word remain similar.
Similar to TextFooler, we use the Universal Sentence Encoder (USE)~\cite{cer2018universal} to compute sentence similarity.
At this step, we only keep synonyms that can maintain sentence similarity score above 0.7.
\textit{(4) Choose a synonym with low confidence as measured by a LM:} At the last step, we choose a replacement word from valid synonyms, that is predicted by the LM with a low probability of $\leq 0.01$. We choose the synonym with the lowest probability if multiple synonyms meet the threshold requirement.
It is possible that less than $N$ words are replaced if the semantic similarity conditions are not met. Empirically, we find that $N=10$ works well in practice, offering a trade-off between evasion rate, and preserving linguistic quality/semantics. We implement \ourattack{} using 2 back-end LMs, namely BERT and GPT2-XL. That said, the backend model is replaceable when more advanced LMs emerge in the future.


% To be more specific, we explain how to find the valid synonym with 4 detailed sub-steps: \textit{1. Synonym Extraction:} This step extracts a candidate set of synonyms for the targeted word as its possible word replacements. \textit{ 2. POS Checking:} This step is to assure that the grammar of the perturbed text remains the same. \textit{3. Semantic Similarity Checking:} This step is to assure that sentence semantic meanings before and after replacing the targeted word remain similar. \textit{4. Choose a low confident synonym via LM:} This step chooses a replacement word that is predicted by the LM with less confidence. 
% (2) In Appendix~\ref{sec:dft_details}, we added a detailed description clarifying how the backend pretrained LM (\eg BERT) identifies a set of words for synonym replacements in \ourattack{}. We put the exact description in the next paragraph for your reading convenience.
% % Specifically, DFTFooler first scans through the whole article via the backend LM, and then ranks each word according to the absolute rank of the prediction probability of its first token/sub-token.~\footnote{For words that are split into multiple tokens, we use the prediction score of the first token in the word. In Figure~\ref{fig:dftfooler}, the prediction confidence of `unicorn' will be the rank of its first subtoken ``uni'', whereas the prediction confidence of `discovered' is the rank of  ``discovered''.}
% (3) We will release the code implementation of the DFTFooler attack once our work gets published.

%  \textit{Appendix~\ref{sec:dft_details} --- Identify a set of important words to be replaced via LM:} \ourattack{} scans a given article to choose the top N confidently predicted words (not token) according to the chosen LM, for replacement. 
% For instance, GPT-2 is a standard left-to-right language model, and for a sequence of tokens \{$x_{1}$, $x_{2}$, ..., $x_{i}$\}, GPT-2 can compute the prediction probability of token $x_{i}$ using Equation~\ref{eqn: language_model}, \ie $P_{x_i}$. We define the absolute rank of $P_{x_i}$ as $R_{x_i}$.
% Given a word $X$, assuming that $X$ can be tokenized by the backend LM (\eg GPT-2) as \{$x_1$, ..., $x_i$\} ($i$ >= 1), the prediction confidence of $X$ will be determined by $R_{x_1}$, where $x_1$ apparently is its token (when $i$ = 1) or its first subtoken.~\footnote{For words that are tokenized into multiple tokens, \ourattack{} only considers the prediction rank of its first subtoken.}


% The reviewer is concerned about the lack of sufficient technical details regarding our proposed adversarial attack \ourattack{}.

% To address this, we made the following changes: (1) In Section~\ref{sec:adaptive-attack-methods}, we better organize and explain critical steps of the \ourattack{} pipeline. 
% To be more specific, we explain how to find the valid synonym with 4 detailed sub-steps: \textit{1. Synonym Extraction:} This step extracts a candidate set of synonyms for the targeted word as its possible word replacements. \textit{ 2. POS Checking:} This step is to assure that the grammar of the perturbed text remains the same. \textit{3. Semantic Similarity Checking:} This step is to assure that sentence semantic meanings before and after replacing the targeted word remain similar. \textit{4. Choose a low confident synonym via LM:} This step chooses a replacement word that is predicted by the LM with less confidence. 
% (2) In Appendix~\ref{sec:dft_details}, we added a detailed description clarifying how the backend pretrained LM (\eg BERT) identifies a set of words for synonym replacements in \ourattack{}. We put the exact description in the next paragraph for your reading convenience.
% % Specifically, DFTFooler first scans through the whole article via the backend LM, and then ranks each word according to the absolute rank of the prediction probability of its first token/sub-token.~\footnote{For words that are split into multiple tokens, we use the prediction score of the first token in the word. In Figure~\ref{fig:dftfooler}, the prediction confidence of `unicorn' will be the rank of its first subtoken ``uni'', whereas the prediction confidence of `discovered' is the rank of  ``discovered''.}
% (3) We will release the code implementation of the DFTFooler attack once our work gets published.

%  \textit{Appendix~\ref{sec:dft_details} --- Identify a set of important words to be replaced via LM:} \ourattack{} scans a given article to choose the top N confidently predicted words (not token) according to the chosen LM, for replacement. 
% For instance, GPT-2 is a standard left-to-right language model, and for a sequence of tokens \{$x_{1}$, $x_{2}$, ..., $x_{i}$\}, GPT-2 can compute the prediction probability of token $x_{i}$ using Equation~\ref{eqn: language_model}, \ie $P_{x_i}$. We define the absolute rank of $P_{x_i}$ as $R_{x_i}$.
% Given a word $X$, assuming that $X$ can be tokenized by the backend LM (\eg GPT-2) as \{$x_1$, ..., $x_i$\} ($i$ >= 1), the prediction confidence of $X$ will be determined by $R_{x_1}$, where $x_1$ apparently is its token (when $i$ = 1) or its first subtoken.~\footnote{For words that are tokenized into multiple tokens, \ourattack{} only considers the prediction rank of its first subtoken.}


% \begin{figure}[!ht]
% \centering
% \includegraphics[width=1.0\columnwidth]{figs/DFTFooler.drawio2.pdf}
% \caption{DFTFooler: Find the most important words.}
% \label{fig:dftfooler_response}
% % \vspace{-3ex}
% \end{figure}

\begin{table}
    %\renewcommand{\arraystretch}{1.2}
    \centering
    %\resizebox{\columnwidth}{!}{%
    %\small{
    \setlength{\tabcolsep}{4pt}
    \setlength\extrarowheight{3pt}  
    \begin{tabular}{c|c|c|c|c}
    \hline
         \multirow{3}{*}{\bf Datasets} & \multicolumn{4}{c}{\bf \makecell{\gltrgpt{} \\Detection Performance (F1)}} 
         \\
         \cline{2-5}
         & \bf  \multirow{2}{*}{\makecell{Before \\ Fine-tuning}}  & \multicolumn{3}{c}{\bf \makecell{\# Samples \\for Fine-tuning}} \\
         \cline{3-5}
         & &\bf 10 &\bf 50 &\bf 100   \\
        %  \cline{2-5}
         \hline
         AI-Writer &1.6 &57.3&59.4&67.5\\
         ArticleForge &44.1&85.2&89.9&92.4\\
         Kafkai &1.0&68.1&72.1&72.6\\
         RedditBot &61.5&92.2&94.3&95.7\\
         \hline
    \end{tabular}
    %}
    \caption{Performance of \gltrgpt{} on \textit{In-the-wild} datasets before and after fine-tuning on \textit{In-the-wild} articles from the real and synthetic classes.
    }
    \label{tab:fine_tune_wild_response}
\end{table}


\noindent \textbf{Major-Rev, Comment-5.} \texttt{``Evaluate the GLTR defense''}

\textit{Response: } 
The reviewer pointed out that we did not consider GLTR when fine-tuning defenses on In-the-wild datasets and suggested re-implementing the logistic regression classifier in Tensorflow to solve the problem.



Fine-tuning as a method for domain adaptation or transfer learning is designed for DNN-based models~\footnote{\url{https://ruder.io/recent-advances-lm-fine-tuning/}}. GLTR does not use a DNN model for classification. 
%Hence, we did not consider it in the traditional fine-tuning experiments. 
Implementing it in TensorFlow does not change the underlying model, and thus it will not in itself make GLTR more adaptable to out-of-distribution data.
Instead, we employ a different strategy---we train a brand new model with limited \textit{In-the-wild} data samples, to achieve domain adaptation for GLTR defenses, and we show that it is reasonably effective. We added these new experiments in Section~\ref{sec:improve-in-the-wild}.
% Previously, we did not consider GLTR as the classifier is not DNN-based, and not suitable for the traditional fine-tuning setting. 

Here are the changes we made: (1) We added ``fine-tuning'' experiments for \gltrgpt{} in Section~\ref{sec:improve-in-the-wild}.
%, but they are, in reality, retraining experiments because the concept of fine-tuning does not exactly apply to logistic classifiers. 
To be more specific, for \gltrgpt{}, we train a new logistic regression model from scratch with 10 \textit{In-the-wild} samples. We then evaluate the trained model on the remaining \textit{In-the-wild} samples. We observe that \gltrgpt{}'s performance recovers significantly as shown in Table~\ref{tab:fine_tune_wild_response}. 
%by \textcolor{blue}{0.55, 0.41, 0.67 and 0.31 F1 Score} on AI-Writer, ArticleForge, Kafkai and RedditBot, respectively. The results are presented in Table~\ref{tab:fine_tune_wild_response}.
(2) To understand how the number of retraining samples impacts \gltrgpt{}'s performance, we additionally conducted experiments with more \textit{In-the-wild} samples (\ie 50 and 100 samples) used for retraining. 
We observe that \gltrgpt{}'s detection performance on \textit{In-the-wild} datasets will only improve with more \textit{In-the-wild} samples used to retrain the detector. Results are presented in Table~\ref{tab:fine_tune_wild_response}. We explained our observation in Finding 3 in Section~\ref{sec:improve-in-the-wild}.
% \jiameng{do we say retrain here?}


% \textit{Response: } 
% This is regarding RevC, Comment-2 in Section~\ref{sec:revc}. The reviewer pointed out that we did not consider GLTR when finetune defenses on In-the-wild datasets and also suggested re-implementing logistic regression classifier in Tensorflow to solve the problem.

% Fine-tuning as a method for domain adaptation or transfer learning is designed for DNN-based models~\footnote{\url{https://ruder.io/recent-advances-lm-fine-tuning/}}. GLTR does not use a DNN model for classification. Hence, we did not consider it in the traditional fine-tuning experiments. Implementing it in TensorFlow does not change the underlying model, and thus it will not in itself make GLTR more adaptable to out-of-distribution data.
% Instead, we employ a different strategy, \ie train a brand new model with limited \textit{In-the-wild} data samples, to achieve domain adaptation for GLTR defenses, and we show that it is reasonably effective.
% % Previously, we did not consider GLTR as the classifier is not DNN-based, and not suitable for the traditional fine-tuning setting. 

% Here are the detailed changes we made: (1) We added ``fine-tuning'' experiments for \gltrgpt{}, but they are, in reality, retraining experiments because the concept of fine-tuning does not exactly apply to logistic classifiers. 
% To be more specific, for \gltrgpt{}, we train a new logistic regression model from scratch with 10 \textit{In-the-wild} samples. We then evaluate the trained model on the remaining \textit{In-the-wild} samples. We observe that \gltrgpt{}'s performance recovers by \textcolor{blue}{0.55, 0.41, 0.67 and 0.31 F1 Score} on AI-Writer, ArticleForge, Kafkai and RedditBot, respectively. The results are presented in Table~\ref{tab:fine_tune_wild_response}.
% (2) To understand how the number of retraining samples impacts \gltrgpt{}'s performance, we additionally conducted experiments with more \textit{In-the-wild} samples (\ie 50 and 100 samples) used for retraining. 
% We observe that \gltrgpt{}'s detection performance on \textit{In-the-wild} datasets will only improve with more \textit{In-the-wild} samples used to retrain the detector. Results are presented in Table~\ref{tab:fine_tune_wild_response}. We explained our observation in Finding 4 in Section~\ref{sec:improve-in-the-wild}.
% % \jiameng{do we say retrain here?}


\noindent \textbf{Major-Rev, Comment-6.} \texttt{``re-implement the logistic regression using the TensorFlow framework and make sure hyperparameters of the logistic regression classifier were carefully tuned''}

\textit{Response: } 
In the previous response (\ie Major-Rev, Comment-5), we discussed why re-implementing the GLTR logistic regression classifier in TensorFlow is not helpful for our setting. In this response, we focus on addressing the concern whether the hyperparameters of logistic regression classifier has been carefully tuned.
%, and also suggested implementing the logistic classifier in Tensorflow.

%We understand that reviewer's concern. 
Previously, we contacted the GLTR authors and used the recommended setting, \ie the default parameter settings of logistic regression in Scikit-learn. We revisited the implementation in Scikit-learn and found that we do not have to re-implement it in Tensorflow to get the classifier properly tuned. For the logistic regression classifier, different optimization solvers, regularization (penalty) and penalty strengths can lead to difference in model performances or convergence. Therefore, we apply grid search on this set of hyperparameters to fit the model during the training. Our results show that grid search did slightly improve the GLTR baseline performances but the improvement is quite limited. We updated the two GLTR detectors (\gltrbert{} and \gltrgpt{}) and reran all the experiments affected by this change. This change required us to rerun 184 experiments in total. We discuss the updated methodology for training GLTR in Section~\ref{sec:six_defenses_info}. Note that this change in training process does not affect any of main takeaways regarding \gltrgpt{} and \gltrbert{}.



More details are here: (1) Instead of using the default setting in Scikit-learn to train the logistic regression classifier (used by the authors of the GLTR paper), we applied grid search to tune hyperparameters during training. For given parameter values, \textit{GridSearchCV}~\cite{gridsearch_cv} in Scikit-learn can exhaustively consider all parameter combinations. We consider a range of values for hyperparameters in logistic regression classifier, \ie ``\textit{solver}'', ``\textit{C}'', ``\textit{penalty}''~\cite{logistic_regression_sk}. (2) Following the above parameter-tuning strategy, we obtained a new \gltrgpt{} detector with 98.5\% F1 score (the previous model without grid search had an F1 score of 96.8\%), and a new \gltrbert{} detector with 79.6\% F1 score (achieved exact similar F1 score compared to the previous model). That said, grid search did slightly improve the GLTR baseline performance, but the improvement is limited.

%(3) We updated two defenses and rerun all the affected experiments throughout the paper. 
% \textit{Response: } 
% This is regarding RevC, Comment-2 and RevC, Comment-5. The reviewer was concerned whether the hyperparameters of logistic regression classifier has been carefully tuned, and also suggested implementing the logistic classifier in Tensorflow.

% We understand that reviewer's concern. 
% Previously, we contacted the GLTR author and used the recommended setting, \ie the default parameter settings of logistic regression in Scikit-learn. We revisited the implementation in Scikit-learn and found that we do not have to re-implement it in Tensorflow to get the classifier properly tuned. For logistic regression classifier, different optimization solvers, regularization (penalty) and penalty strengths can lead to difference in model performances or convergence. 
% Therefore, we apply grid search on this set of hyperparameters to fit the model during the training. Our results show that grid search did slightly improve the GLTR baseline performances but the improvement is quite limited. We updated two detectors and rerun all evaluations affected by this change. This change required us to rerun 184 experiments in total.


% Here are the detailed changes we made: (1) Instead of using the default setting in Scikit-learn to train the logistic regression classifier (used by the authors of the GLTR paper), we applied grid search to tune hyperparameters during training. For given parameter values, \textit{GridSearchCV}~\cite{gridsearch_cv} in Skicit-learn can exhaustively consider all parameter combinations. We consider a range of values for hyperparameters in logistic regression classifier, \ie ``\textit{solver}'', ``\textit{C}'', ``\textit{penalty}''~\cite{logistic_regression_sk}. We carefully explained our experimental settings in the paper. (2) Following the above parameter-tuning strategy, we obtained a new \gltrgpt{} detector with 98.5\% F1 score (the previous model without grid search had an F1 score of 96.8\%), and a new \gltrbert{} detector with 79.6\% F1 score (achieved exact similar F1 score compared to the previous model). That said, grid search did slightly improve the GLTR baseline performance but the improvement is quite limited.
% (3) We updated two defenses and rerun all the affected experiments throughout the paper. Note that this change in training process does not affect any of main takeaways regarding \gltrgpt{} and \gltrbert{}.



\noindent \textbf{Major-Rev, Comment-7}
\texttt{``clarify several claims made in the experiments: (a) see review D points 2 and 3, (b) Explain how in Table IV, after fine-tuning the GROVER (unidirectional model) outperforms BERT-Defense (Bidirectional model)''}

%%%%%%%%%%%%%%Roberta GRUEN CDF%%%%%%%%%%%%%%%

\begin{figure}[!t]
\centering
\includegraphics[width=0.95\columnwidth]{figs/ROBERTA_CDF_5curves.pdf}
%\vspace{-2ex}
\caption{The CDF of GRUEN score on perturbed text produced by different adversarial perturbation methods, 
\ie \ourattack{}, random perturbations, and TextFooler, based on attacking \rbert{} (in Table~\ref{tab:adversarial_perturbs_results}).}
%\vspace{-4ex}
\label{fig:ROBERTA_CDF_5curves_response}
\end{figure}
%%%%%%%%%%%%%%Roberta GRUEN CDF%%%%%%%%%%%%%%%


\textit{Response: } 
This covers 3 comments from Reviewers. We explain how we addressed each of the comments below.
%Specifically, (a) is regarding RevD, Comment-2 and RevD, Comment-3, and (b) is regarding RevC, Comment-6. 

%\textbf{(1) RevD, Comment-2}:
(1) Reviewer D made the following comment: \textit{``Some claims seem not convincing. Please clarify. For instance, when comparing the adversarial examples, the authors claimed that “DFTFooler also outperforms the random perturbation scheme for all defenses.” This does not match the results shown in Table VII. In Table VII, DFTFooler with BERT backend achieves marginally higher ER than random perturbation. However, its GRN-AFTER is lower than random perturbation. This may not mean DFTFooler is better considering the trade-off. Moreover, DFTFooler with GPT2-XL backend even has lower ER than random perturbation.''}

% \bimal{Jiameng, I updated. please read again.}
Results relevant to this comment are in Table~\ref{tab:adversarial_perturbs_results} in our revised draft. A major change in this revision is that we make the context window size of each defense uniform in size \ie 512 tokens. (We made this change due to the Major-Rev, Comment-9, discussed later in this section). Since adversarial attacks are expected to perturb words within the context window, we need to rerun all the adversarial attack experiments for \gbert{}, \gltrgpt{}, and \grover{}, for which the context window size has changed. We reran all the adversarial attack experiments for the above defenses and updated the results in Table~\ref{tab:adversarial_perturbs_results}. We also found and fixed a bug in our random perturbation attack causing the perturbations to not be entirely random.
With the updated evaluation results, we need to clarify 3 points: \textit{(a) Despite what the reviewer observed in our previous submission, in our new results, we observe that DFTFooler with both BERT and GPT-2 backend outperforms the random perturbation attack for all the defenses.} 
Specifically, DFTFooler with BERT backend show significant percentage increase in ER (Evasion Rate) ranging from 35.8\% to 95.0\% compared to random perturbations,
while DFTFooler with GPT2-XL backend show percentage increase in ER ranging from 18.8\% to 73.5\% compared to random perturbations. 
(b) Note that, unlike TextFooler, DFTFooler achieves such attack performance rates without a single query to the victim classifier. (c) The average GRUEN scores of samples with random perturbations are comparable to the GRUEN scores of \ourattack{} with GPT2-XL backend---across all defenses, the average absolute difference between GRUEN scores is only 0.014. Figure~\ref{fig:ROBERTA_CDF_5curves_response} shows how close the GRUEN score distributions are for DFTFooler, and random perturbation attack.


% \textbf{(1) RevD, Comment-2}:
% To quote RevD, Comment-2: \textit{``Some claims seem not convincing. Please clarify. For instance, when comparing the adversarial examples, the authors claimed that “DFTFooler also outperforms the random perturbation scheme for all defenses.” This does not match the results shown in Table VII. In Table VII, DFTFooler with BERT backend achieves marginally higher ER than random perturbation. However, its GRN-AFTER is lower than random perturbation.  This may not mean DFTFooler is better considering the trade-off. Moreover, DFTFooler with GPT2-XL backend even has lower ER than random perturbation.''}

% The reviewer is referring to results in Table~\ref{tab:adversarial_perturbs_results} in the revision. A major change in this revision is that we make the context window size of each defense uniform in size \ie 512 tokens. (We made this change due to the Major-Rev, Comment-9 in Section~\ref{sec:mjrev}). Since adversarial attacks are suppose to perturb words within the context window, we need to rerun all the adversarial attack experiments for \gbert{}, \gltrgpt{}, and \grover{}, of which the context window size has been changed. Therefore,
% We rerun all the adversarial attack experiments for the above defenses and updated all the results in Table~\ref{tab:adversarial_perturbs_results}. With the updated evalaution results, we need to clarify 2 points: \textit{(1) Despite what the reviewer observed in our previous submission, after we rerun the experiments, we observe that DFTFooler with both BERT and GPT-2 backend outperform the random perturbation attack for all the defenses.} 
% Specifically, DFTFooler with BERT backend show significant percentage increase in ER (Evasion Rate) ranging from 35.8\% to 95.0\% compared to random perturbation,
% while DFTFooler with GPT2-XL backend show percentage increase in ER ranging from 18.8\% to 73.5\% compared to random perturbation. 
% (2) Note that, unlike TextFooler, DFTFooler achieves such attack performance rates without a single query to the victim classifier, which is a more challenging attack. \textcolor{blue}{Figure~\ref{fig:ROBERTA_CDF_5curves_response} shows how close the GRUEN score distributions are for DFTFooler, TextFooler and random perturbation attack.} 



% %%%%%%%%%%%%%%%%%%%%
(2) Reviewer D made the following comment: ``\textit{Some explanations for some findings are unhelpful. For instance, `Defenses trained on conditionally generated text are not able to detect unconditionally generated text.' Is there any explanation why this happens?}''

Reviewer D is talking about Finding 6 in the updated draft. To address the concern, we provided an explanation under Finding 6 in Section~\ref{sec:adaptive-attack-eval}. 

This is our explanation: \gbert{} which is originally trained on conditionally generated text (with a single priming token), shows over 47.7\% degradation in $\Delta$R when tested on unconditionally generated text (\ie with 0 priming tokens). 
All the other defenses are trained on unconditionally generated text, and shows significantly less degradation, compared to \gbert{}. 
We believe that this is because defenses trained on conditionally generated text learn a narrow distribution of synthetic text. 
We can think of LMs as being in a particular state space at each time-step. The priming tokens might lead the model into a particular state space which the model might not have reached on its own due to those `priming tokens' being low probability tokens, and thus less likely to be sampled in an unconditional setting. Therefore, conditionally trained models might learn a different and narrower distribution of synthetic text and not generalize well to unconditionally generated text. 



%We believe that this is because defenses trained on conditionally generated text learn a narrow distribution of synthetic text because language models are conditional probability models and an initial priming token can alter the distribution of the generated text. We can think of LMs as being in a particular state space at each time-step. If the priming tokens lead the model into a particular state space which the model might not have reached on it’s own due to those ‘priming tokens’ being low probability tokens, and thus less likely to be sampled in an unconditional setting, then conditionally trained models might learn a narrower distribution of synthetically generated text and not generalize well to unconditionally generated text. 

% \textbf{RevD, Comment-3}: To Quote RevD, Comment-3, ``\textit{Some explanations for some findings are unhelpful. For instance, `Defenses trained on conditionally generated text are not able to detect unconditionally generated text.' Is there any explanation why this happens?}''

% The reviewer D is concerned about the explanation of the Finding 6 in the revision. To address the concern, we provided a detailed explanation under Finding 6 in Section~\ref{sec:adaptive-attack-eval}. This is our explanation: We believe that this is because defenses trained on conditionally generated text learn a narrow distribution of synthetic text because language models are conditional probability models and an initial priming token can alter the distribution of the generated text. We can think of LMs as being in a particular state space at each time-step. If the priming tokens lead the model into a particular state space which the model might not have reached on it’s own due to those ‘priming tokens’ being low probability tokens, and thus less likely to be sampled in an unconditional setting, then conditionally trained models might learn a narrower distribution of synthetically generated text and not generalize well to unconditionally generated text. 

%%%%%%%%%%%%%%%

 (3) Reviewer C made the following comment: ``\textit{In finding 2, the authors stated that bidirectional models if robustly trained perform better than unidirectional models. But according to Table IV, after fine-tuning the GROVER (unidirectional model) outperforms BERT-Defense (Bidirectional model). How can the authors explain this?}'' 
 
 The reviewer is referring to the Finding 2 in the revised draft, \ie \textit{``Robustly pre-trained bidirectional models generalize better than unidirectional models.''}. We want to clarify a few things: (a) There seems to be some confusion about which model we were referring to in this finding. To quote from the paper, we wrote, “Robustly pre-trained bidirectional models generalize better than unidirectional models” and this was referring to the RoBERTa-Defense. ‘Robustly pre-trained’ is a reference to the meaning of RoBERTA which is “Robustly optimized BERT”. We stated this because we observed that the RoBERTa-Defense actually performed better on the In-the-wild datasets than it did on the baseline test dataset. (b) This finding is not related to the fine-tuning experiments in Table~\ref{tab:fine_tune_wild} which shows results for BERT-Defense, and not RoBERTa. 

To address this concern, we modified our statement of the finding as ``\textit{Robustly pre-trained bidirectional models, \ie RoBERTa, generalize better than unidirectional models.}'' to avoid the confusion.

% \textbf{RevC, Comment-6}:
%  To Quote RevC, Comment-6, ``\textit{In finding 2, the authors stated that bidirectional models if robustly trained perform better than unidirectional models. But according to Table IV, after fine-tuning the GROVER (unidirectional model) outperforms BERT-Defense (Bidirectional model). How can the authors explain this?}'' 
 
%  The reviewer is referring to the Finding 2 in the revision ---" ``\textit{Robustly pre-trained bidirectional models generalize better than unidirectional models.}'' We want to clarify: (1) There seems to be some confusion about which model we were referring to in this finding. To quote from the paper, we wrote, “Robustly pre-trained bidirectional models generalize better than unidirectional models” and this was referring to the RoBERTa-Defense. ‘Robustly pre-trained’ was a reference to the meaning of RoBERTA which is “Robustly optimized BERT”. We stated this finding because we observed that the RoBERTa-Defense actually performed better on the In-the-wild datasets than it did on the baseline test dataset. (2) This finding is not related to the fine-tuning experiments in Table~\ref{tab:fine_tune_wild} which shows results for BERT-Defense, and not RoBERTa. 

% To address this concern, we modified our statement of the finding as ``\textit{Robustly pre-trained bidirectional models, \ie RoBERTa, generalize better than unidirectional models.}'' to avoid the confusion.


\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.48\columnwidth}
  \includegraphics[width=\columnwidth]{figs/FAST_perturb_token_ER1.pdf}
\caption{Attack \fast{}.}
\label{fig:fast_perturb_response}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.48\columnwidth}
  \includegraphics[width=\columnwidth]{figs/BERT_perturb_token_ER1.pdf}
\caption{Attack \gbert{}.}
\label{fig:gbert_perturb_response}
\end{subfigure}
% \vspace{0.1in}
\caption{Evasion rate and average GRUEN score of perturbed text achieved by \ourattack{} and random perturbations when attacking \fast{} (a) and \gbert{} (b), based on 5, 10, 15, 20 word perturbations.}
% \vspace{-0.1in}
\label{fig:word_perturb_plot_response}
\end{figure}
 
 
 %%%%%%%%%%%%%%baseline_token_length%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\includegraphics[width=0.9\columnwidth]{figs/all_defenses_token_length.pdf}
\caption{Detection performances of the defenses with different context window sizes, \ie 64, 128, 256, 512 tokens.}
\label{fig:baseline_token_length_response}
\end{figure}
%%%%%%%%%%%%%%baseline_token_length%%%%%%%%%%%%%%%

\noindent \textbf{Major-Rev, Comment-8.} \texttt{``an analysis of the number of tokens used for perturbations''}

\textit{Response: } 
The reviewer suggests to analyze how the number of perturbations in our adversarial attack can influence evasion rate. In our previous submission, we limited the number of perturbations to 10.

To address the concern, we experimented with different numbers of perturbations made to the text. We observe that there is a trade-off between Evasion Rate and preservation of text quality (GRUEN score). 
%\textcolor{blue}{as well as overall stealthiness of the attack}. 
We made the following changes: (1) We do this experiment for \gbert{} and \fast{}. We vary the number of word perturbations by 5, 10, 15, 20 used in \ourattack{} and the random perturbation attack. The results are presented in Figure~\ref{fig:word_perturb_plot_response}. (2) We explain our observation in Section~\ref{sec:adaptive-attack-eval}. While the Evasion Rate (ER) is higher with more perturbations, the text quality, as indicated by the GRUEN metric, tends to degrade. Therefore, there is a trade-off between Evasion Rate and preservation of text quality. In order to make a reasonable trade off between the attack performance and preserving text quality, we limited the number of word perturbations to 10.

%  \textit{Response: } 
% This is regarding RevC, Comment-8 in Section~\ref{sec:revc}, which suggests to analyze how number of perturbations in our adversarial attacks can influence evasion rate. In our previous submission, we limited the number of perturbations to 10.

%  To address the concern, we experimented with different numbers of total perturbations made to the text. We observe there is a trade-off between Evasion Rate and preservation of text quality (GRUEN score) \textcolor{blue}{as well as overall stealthiness of the attack}. 

% Here are the detailed changes we made: (1) \textcolor{blue}{Of the 6 defenses, we chose 2 representative defenses - \gbert{} and \fast{} - } and varied the number of word perturbations by 5, 10, 15, 20 used in \ourattack{} and the random perturbation attack. The results are presented in Figure~\ref{fig:word_perturb_plot_response}. (2) We explained our observation in Section~\ref{sec:adaptive-attack-eval}. That is, while the Evasion Rate (ER) was higher with more perturbations, the text quality, as indicated by the GRUEN metric, tends to degrade. Therefore, there is a trade-off between Evasion Rate and preservation of text quality \textcolor{blue}{as well as overall stealthiness of the attack}. In order to make a reasonable trade off between the attack performance and stealthiness, we limited the number of perturbations to 10.



\begin{table*}
    %\renewcommand{\arraystretch}{1.2}
    \centering
    %\resizebox{\columnwidth}{!}{%
    %\small{
    \setlength{\tabcolsep}{3pt}
    \setlength\extrarowheight{3pt}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \hline
         \multirow{3}{*}{\bf Datasets} & 
         \multicolumn{10}{c}{\bf Length (\# of Tokens) of Test Sets Under Detection} \\
         \cline{2-11}
         &\multicolumn{2}{c|}{\bf \gbert{}} &
         \multicolumn{2}{c|}{\bf \gltrbert{}} &
         \multicolumn{2}{c|}{\bf \gltrgpt{}} &
         \multicolumn{2}{c|}{\bf \grover{}} &
         \multicolumn{2}{c}{\bf \fast{}/\rbert{}} \\
         \cline{2-11}
         & \bf  Mean  & \bf Median& \bf Mean & \bf Median &\bf Mean &\bf Median& \bf Mean & \bf Median &\bf Mean &\bf Median  \\
         \cline{2-11}
         \hline
         Real &391&512&390&512&474&512&367&461&462&512\\
         Synthetic &406&512&398&512&468&512&411&512&453&512\\
         \hline
    \end{tabular}
    %}
    \caption{Median and mean lengths (\# of tokens) of articles within the context window used by the defenses for evaluation.
    }
    \label{tab:token_len_mean_median}
\end{table*}
 


\noindent \textbf{Major-Rev, Comment-9.} \texttt{``study whether length of documents matter in detection''}

\textit{Response: } 
% \bimal{Jiameng: please read and check.}
The reviewer is asking: (1) whether the synthetic document lengths and the real document lengths in our evaluation are roughly similar or not, and (2) whether the length of documents matters in detection.

First, we want to clarify that lengths of real and synthetic documents used in detection are roughly similar. To further address both points, we made the following change to the defense evaluation configuration. Previously, the defenses used different context window sizes (we borrowed the settings from their original work), \ie 192 tokens for \gbert{}, 1024 tokens for \grover{} and \gltrgpt{}, and 512 tokens for the other 3 defenses. To eliminate any impact of varying context window sizes used for detection, we changed the context window size to a uniform size for all defenses---\textit{we now use the first 512 tokens of an article as the context window for detection}. This change required us to rerun more than 200 experiments throughout the paper. This change did result in slight performance fluctuations, but our main findings generally remain the same. While, making this change in context window configuration, we identified an error in our \grover{} configuration---\grover{} was applied to a context window at the end of the article, even though it was trained on text at the beginning of the article (in its context window). We fixed this configuration error, and thoroughly re-checked all our defense configurations. This correction actually fixed the performance degradation issue we observed when we apply \grover{} to text in the wild, \ie \grover{} now generalizes better to In-the-wild datasets (Table~\ref{tab:eval_in_the_wild}).


We provide more details below:\\
\textit{How does length of the context window impact detection?}
To understand this, we additionally evaluated the defenses using various context window sizes, \ie 64, 128, 256, and 512 tokens. Results are shown in Figure~\ref{fig:baseline_token_length_response}. Performance (F1 score) monotonically increases as the context window size increases. Therefore, we chose a 512 token window size. Larger window size would significantly increase computational complexity for all experiments, and some pre-trained models only support a certain maximum window size (\eg 512 tokens for BERT). We added this discussion in Section~\ref{sec:six_defenses_info}.

%We observe a linear trend for all defenses that the evaluation performance will monotonically improve as the context window size under detection increases.
 
\textit{Lengths of the real and synthetic articles used for detection are similar.} For all our defenses, the detection is based on the first 512 tokens at the beginning of the article. So regardless of the length of the original article, detection is only based on the length of the article within the classifier’s context window. Table~\ref{tab:token_len_mean_median} shows the median and mean length (\# of tokens) of articles within the context window used by the defenses for test sets evaluated in Table~\ref{tab:defenses-setup}. This indicates that the lengths (\# of tokens) of real and synthetic articles are roughly similar. Hence length differences do not impact any of our current findings. 

% Here are the detailed explanations/changes:
% (1) Each defense has a pre-defined context window --- \eg \rbert{} uses a context window of the first 512 tokens in an article for detection. Note that these tokens are not words, but sub-words as determined by the tokenization scheme. So regardless of the length of the original article, detection is only based on the length of the article within the classifier’s context window. 
% % We understand why this question came up. Table~\ref{tab:in_the_wild_details} in our previous submission shows the full lengths of articles (as number of words, not tokens), which is not the length within the context window. We have removed this information from the table to avoid confusion. 
% Table~\ref{tab:token_len_mean_median} below shows the median and mean length (\# of tokens) of articles within the context window used by the defenses for test sets evaluated in Table~\ref{tab:defenses-setup}. This indicates that the lengths (\# of tokens) of real and synthetic articles are roughly similar. Hence length differences do not impact any of our findings. 
% (2) In this revision, we set the first 512 tokens as the uniform context window size used for discrimination for all the defenses. 
% New baseline detection performance based on 512 tokens are presented in Table~\ref{tab:defenses-setup}. 
% We also updated all the experiments affected by this change throughout the paper. Despite the slight performance fluctuation, our main findings do not change. 
% (3) Additionally, we evaluated all the defenses against various context window sizes, \ie 64, 128, 256, 512 tokens. New evaluation results are presented in Figure~\ref{fig:baseline_token_length_response}.
% We observe a linear trend for all defenses that the evaluation performance will monotonically improve as the maximum token length under detection increases. This is in line with the findings in ~\cite{ippolito2019human}.


% \textit{Response: } This is regarding RevA, Comment-4 in Section~\ref{sec:reva}. The reviewer was concerned about (1) whether the synthetic document lengths and the real document lengths in our evaluation are roughly similar or not. (2) whether the length of documents matter in detection.

%  (1) For the first concern, we want to clarify that lengths of real and synthetic documents used in detection are roughly similar. We explain more details in the next paragraph. (2) To address the second concern, we made a major change to the paper. Previously, all 6 defenses have different pre-defined context window sizes, which are the original settings (\eg 192 tokens for \gbert{}, 1024 tokens for \grover{} and \gltrgpt{}). To eliminate the impact of document lengths in detection, we changed the context window size to a uniform size, \ie the first 512 tokens. This change requires us to rerun more than 200 experiments in throughout the paper. This change did result in slight performance fluctuation, but our previous main findings generally remain the same. (3) Besides, we additionally evaluated the defenses against various context window sizes, \ie 64, 128, 256, 512 tokens. We observe a linear trend for all defenses that the evaluation performance will monotonically improve as the context window size under detection increases.
 
% Here are the detailed explanations/changes:
% (1) Each defense has a pre-defined context window --- \eg \rbert{} uses a context window of the first 512 tokens in an article for detection. Note that these tokens are not words, but sub-words as determined by the tokenization scheme. So regardless of the length of the original article, detection is only based on the length of the article within the classifier’s context window. 
% % We understand why this question came up. Table~\ref{tab:in_the_wild_details} in our previous submission shows the full lengths of articles (as number of words, not tokens), which is not the length within the context window. We have removed this information from the table to avoid confusion. 
% Table~\ref{tab:token_len_mean_median} below shows the median and mean length (\# of tokens) of articles within the context window used by the defenses for test sets evaluated in Table~\ref{tab:defenses-setup}. This indicates that the lengths (\# of tokens) of real and synthetic articles are roughly similar. Hence length differences do not impact any of our findings. 
% (2) In this revision, we set the first 512 tokens as the uniform context window size used for discrimination for all the defenses. 
% New baseline detection performance based on 512 tokens are presented in Table~\ref{tab:defenses-setup}. 
% We also updated all the experiments affected by this change throughout the paper. Despite the slight performance fluctuation, our main findings do not change. 
% (3) Additionally, we evaluated all the defenses against various context window sizes, \ie 64, 128, 256, 512 tokens. New evaluation results are presented in Figure~\ref{fig:baseline_token_length_response}.
% We observe a linear trend for all defenses that the evaluation performance will monotonically improve as the maximum token length under detection increases. This is in line with the findings in ~\cite{ippolito2019human}.

%%%%%%%%%%%%% NEW finetuning experiments
\begin{table}
    \centering
    \setlength{\tabcolsep}{3pt}
    \setlength\extrarowheight{3pt}
    \begin{tabular}{c|c|c|c|c}
    \hline
    \bf \multirow{4}{*}{\bf{Defenses}} & \multicolumn{4}{c}{\multirow{2}{*}{\bf{\makecell{Detection Performance(Recall) \\ with Adversarial Training}}}}\\ \\
    \cline{2-5} &\multirow{2}{*}{\bf{\makecell{  Adaptive \\Attack}}} & \multirow{2}{*}{\bf\makecell{Recall \\ Before}} & \multirow{2}{*}{\bf \makecell{Recall \\After}} &\multirow{2}{*}{\bf $\Delta$R}\\
    &&&&\\
    \hline
        %  \gbert{}&priming token 0&0.86&0.45&0.86\\
        \gbert{}&Priming Token 0&44.9&85.8&+91.0\\
        %  \gltrgpt{} &Top k 160&0.98&0.43& 0.99 \\
        \gltrgpt{} &Top-k 160&42.8& 99.2&+131.7 \\
        %  \grover{}&Top p 1&0.91&0.59&0.77\\
        \grover{}&Top-p 1.0&58.7&77.5&+32.0\\
         \hline
    \end{tabular}
    %}
    \caption{ Detection performance (Recall) of defenses (\gbert{}, \gltrgpt{}, \grover{}) fine-tuned to their most effective adaptive attack setting as indicated. $\Delta$R is percentage change of Recall from Recall before training to Recall after training.
    }
    \label{tab:fine_tune_decoding_response}
\end{table}
%%%%%%%%%%%% NEW finetuning experiments

\noindent \textbf{Major-Rev, Comment-10.} \texttt{``evaluate if the performance of the detectors is as good as advertised if the defense is optimally fine-tuned to the synthetic text generation procedure''}

\textit{Response: } 
 The reviewer is asking about the performance of detectors if they are optimally fine-tuned towards an attack strategy. To address this, conducted additional experiments and explain our findings in a subsection titled ``Adversarial training to enable robustness against adaptive attacks'' in Section~\ref{sec:towards_adv_robustness}.
 
 We replicate the text from that section here:\\
 We investigate whether a defender can recover from an adaptive attack via \textit{adversarial training}, \ie by training a defense on a set of known adversarial samples to build resilience against similar adversarial samples. We start by studying recovery from adaptive attacks that change the text generation process. We fine-tune \gbert{}, \grover{} and \gltrgpt{}~\footnote{Since \gltrgpt{} is not DNN-based, we instead train a new \gltrgpt{} model from scratch with samples generated under the attack setting.} on new samples generated from their most effective adaptive attack setting (Tables~\ref{tab:decoding_eval_short} and~\ref{tab:priming_eval_short}). We use 1,000 new articles each for both the synthetic and real class for adversarial training. We then evaluate the adversarially trained models against their original adaptive attack dataset. As shown in Table~\ref{tab:fine_tune_decoding_response}, we observe that the fine-tuned \gbert{}, \gltrgpt{} and \grover{} achieve 91.0\%, 131.7\% and 32.0\% increase in $\Delta$R, respectively. Therefore, the fine-tuned models are able to recover from the attack.

Next, we explore adversarial training to recover from our \ourattack{} attack. We use \rbert{} for this experiment. From our dataset of 1,000 adversarial samples from \ourattack{}, we use a random set of 500 samples for adversarial fine-tuning, and test the adversarially trained \rbert{} on the remaining 500 adversarial samples. \ourattack{} becomes ineffective as its evasion rate drops from 51.4\% on \rbert{} (in Table~\ref{tab:adversarial_perturbs_results}) to 1.6\% on the adversarially fine-tuned \rbert{}. 

This indicates that fine-tuning or optimizing the defense towards a specific attack is a way forward, but the defender may have to frequently adapt their defenses against newer adaptive strategies or their variants. On the other hand, by using robust semantic features, one can potentially build in resilience in an attack-agnostic way.


% Under a realistic detection scenario, the defender has limited or no a priori knowledge about synthetic text generation procedure in the wild. For example, when collecting data from text-generation services, \textcolor{blue}{we only knew that models from the Transformer family were being used.}
% Our goals (stated in Section~\ref{sec:background}) focus on understanding and improving performance in the wild, and also understanding performance against adaptive attackers. 
% To address this concern, we optimally finetuned defenses (\gbert{}, \gltrgpt{} and \grover{}) to particular settings that they suffer from, we observe an obvious bounce-back in their F1 score. 
% % (\jiameng{as good as advertised?}) 
% That said, the defender may have to frequently adapt their defenses against new attack strategies. We present our experiment results in Table~\ref{tab:fine_tune_decoding_response}, and our observation under title \textit{``Adversarial training to enable robustness against adaptive attacks''} in Section~\ref{DistilFAST}. 

% Here are the detailed changes we made: (1) We optimally fine-tune defenses towards the most effective decoding setting or priming token setting in Table~\ref{tab:decoding_eval_short} and Table~\ref{tab:priming_eval_short}, and we re-evaluate the fine-tuned defense under the same attack. To be more specific, we selected 3 most effective attack scenarios: \gbert{} under the \textit{0 priming token} attack, \gltrgpt{} under the \textit{Top-k 160} attack, \grover{} under the \textit{Top-p 1.0} attack. For each scenario, we fine-tuned the defense with 1,000 synthetic samples generated from the corresponding decoding/priming setting and re-evaluate the fine-tuned defense against the same attack dataset. 
% For instance, in Scenario 1, we first finetune \gbert{} with 1k synthetic samples generated under 0 priming token and then evaluate the fine-tuned \gbert{} on the previous attack dataset (4k real text vs 4k synthetic text generated from 0 priming token).
% \textcolor{blue}{Since we were not able to finetune \gltrgpt{} as the way we do for \gbert{} and \grover{}, we instead retrain a new logistic regression classifier with 1,000 synthetic samples.}
% (2) In Table~\ref{tab:fine_tune_decoding_response}, we observe that the finetuned defenses achieve +91.0\%, +131.7\% and +32.0\% in $\Delta$R for \gbert{}, \gltrgpt{} and \grover{}, respectively. This indicates that fine-tuning the defense towards a specific attack is a way forward, but the defender may have to frequently adapt their defenses against new attack strategies.



% \textit{Response: } 
% This is regarding RevA, Comment-2 in Section~\ref{sec:reva}. The reviewer is curious about the performance of detectors optimally finetuned to a particular decoding/priming setting of the synthetic text generator.

% Under a realistic detection scenario, the defender has limited or no a priori knowledge about synthetic text generation procedure in the wild. For example, when collecting data from text-generation services, \textcolor{blue}{we only knew that models from the Transformer family were being used.}
% Our goals (stated in Section~\ref{sec:background}) focus on understanding and improving performance in the wild, and also understanding performance against adaptive attackers. 
% To address this concern, we optimally finetuned defenses (\gbert{}, \gltrgpt{} and \grover{}) to particular settings that they suffer from, we observe an obvious bounce-back in their F1 score. 
% % (\jiameng{as good as advertised?}) 
% That said, the defender may have to frequently adapt their defenses against new attack strategies. We present our experiment results in Table~\ref{tab:fine_tune_decoding_response}, and our observation under title \textit{``Adversarial training to enable robustness against adaptive attacks''} in Section~\ref{DistilFAST}. 

% Here are the detailed changes we made: (1) We optimally fine-tune defenses towards the most effective decoding setting or priming token setting in Table~\ref{tab:decoding_eval_short} and Table~\ref{tab:priming_eval_short}, and we re-evaluate the fine-tuned defense under the same attack. To be more specific, we selected 3 most effective attack scenarios: \gbert{} under the \textit{0 priming token} attack, \gltrgpt{} under the \textit{Top-k 160} attack, \grover{} under the \textit{Top-p 1.0} attack. For each scenario, we fine-tuned the defense with 1,000 synthetic samples generated from the corresponding decoding/priming setting and re-evaluate the fine-tuned defense against the same attack dataset. 
% % For instance, in Scenario 1, we first finetune \gbert{} with 1k synthetic samples generated under 0 priming token and then evaluate the fine-tuned \gbert{} on the previous attack dataset (4k real text vs 4k synthetic text generated from 0 priming token).
% \textcolor{blue}{Since we were not able to finetune \gltrgpt{} as the way we do for \gbert{} and \grover{}, we instead retrain a new logistic regression classifier with 1,000 synthetic samples.}
% (2) In Table~\ref{tab:fine_tune_decoding_response}, we observe that the finetuned defenses achieve +91.0\%, +131.7\% and +32.0\% in $\Delta$R for \gbert{}, \gltrgpt{} and \grover{}, respectively. This indicates that fine-tuning the defense towards a specific attack is a way forward, but the defender may have to frequently adapt their defenses against new attack strategies.



% Our results indicate that fine-tuning the defense towards a specific attack is a way forward, but the defender may have to frequently adapt their defenses against new attack strategies.


\noindent \textbf{Major-Rev, Comment-11.} \texttt{``Open-source dataset''}

\textit{Response: } As we mentioned at the end of the introduction section, we will release the real-world synthetic datasets to the research community. We will also release the code for our adversarial attack tool \ourattack{}.
%, as well as any other critical resources that can help fellow researchers in the community.


\subsection{Response to Review A}
\label{sec:reva}
% \subsubsection{Detailed Review Comments}
% \newline

\begin{table*}
    %\renewcommand{\arraystretch}{1.2}
    \centering
    %\resizebox{\columnwidth}{!}{%
    %\small{
    \setlength{\tabcolsep}{4pt}
    \setlength\extrarowheight{4pt}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
    \hline
         \multirow{4}{*}{\bf Datasets} &
         \multicolumn{12}{c}{\bf Detection Performance (F1)}\\
         \cline{2-13}
         &\multicolumn{4}{c|}{\bf \gbert{}} & \multicolumn{4}{c|}{\bf \gltrgpt{}} & \multicolumn{4}{c}{\bf \grover{}} \\
         \cline{2-13}
         & \multirow{2}{*}{\bf \makecell{Before \\ Fine-tuning}} & \multicolumn{3}{c|}{\bf \makecell{\# Samples\\for Fine-tuning}} & 
          \multirow{2}{*}{\bf \makecell{Before \\ Fine-tuning}} &
         \multicolumn{3}{c|}{\bf \makecell{\# Samples\\for Fine-tuning}} & 
         \multirow{2}{*}{\bf \makecell{Before \\ Fine-tuning}} &
         \multicolumn{3}{c}{\bf \makecell{\# Samples\\for Fine-tuning}}\\
          \cline{3-5}
          \cline{7-9}
          \cline{11-13}
         &&\bf 10&\bf 50&\bf 100&&\bf 10&\bf 50&\bf 100&&\bf 10&\bf 50&\bf 100\\
        %  & \bf  F1-B  & \bf F1-A1& \bf F1-A2 & \bf F1-A3 &\bf F1-B &\bf F1-A1& \bf F1-A2 & \bf F1-A3 &\bf F1-B &\bf F1-A1 & \bf F1-A2 & \bf F1-A3  \\
        %  \cline{2-13}
        %  &&&&&&&&&&&&\\
         \cline{2-13}
         \hline
         AI-Writer & 28.8&68.9&85.8&90.4&1.6&57.3&59.4&67.5&87.6&90.7&93.8&94.8\\
         ArticleForge &19.7&85.3&90.8&93.7&44.1&85.2&89.9&92.4&76.9&86.5&95.9&97.1\\
         Kafkai &65.9&71.0&83.8&85.0&1.0&68.1&72.1&72.6& --&--&--&--\\
         RedditBot &14.1&71.5&90.6&95.2&61.5&92.2&94.3&95.7&--&--&--&--\\
         \hline
    \end{tabular}
    %}
    \caption{Detection performance in F1 (\%) of \gbert{}, \gltrgpt{} and \grover{} on \textit{In-the-wild} datasets before and after fine-tuning on a limited set of articles
    from the real and synthetic classes. 
    ``--'' represents experiments we ignored: We did not fine-tune \grover{} on non-news domain datasets, \ie Kafkai and RedditBot. This is because \grover{} is only trained for the news domain.
    }
    \label{tab:fine_tune_wild_long_response}
\end{table*}


\noindent \textbf{RevA, Comment-1.} \texttt{``Note that here I largely discard the experiments of section 4.B that fine-tune the detector because only 10 samples are used for this. In fact, I believe this is a significant weakness of the paper. The problem is that the case with more samples is not evaluated so we have no way of knowing the detector's performance with 100 or 1000 samples.''}

\textit{Response:} When we chose a sample size of 10 for fine-tuning, our intention was to consider a more realistic detection scenario, as it is harder to obtain ground-truth for attack data (synthetic samples) than benign data. 

To address this concern, we further evaluated the defenses with a larger number of fine-tuning samples, \ie 50 and 100 \textit{In-the-wild} samples. The detection performances after fine-tuning the detector are presented in Table~\ref{tab:fine_tune_wild_long_response}. We found that detection performance will only improve if more samples are used for fine-tuning. This is generally the case when a DNN is fine-tuned on a larger number of samples from the new distribution/domain. We added this discussion in Section~\ref{sec:improve-in-the-wild}. 

% \textit{Response:} When we chose a sample size of 10, our intention was to consider a more realistic detection scenario, as it is harder to obtain ground-truth for attack data (synthetic samples) than benign data. 

% To address this concern, we further evaluated the defenses with a larger number of fine-tuning samples, \ie 50 and 100 \textit{In-the-wild} samples. We found that detection performance will only improve if more samples are used for fine-tuning. This is generally the case when a DNN is fine-tuned on a larger number of samples from the new distribution/domain. We added this discussion under Finding 3 in Section~\ref{sec:improve-in-the-wild}. The detection performances after fine-tuning the detector are presented in Table~\ref{tab:fine_tune_wild_long_response}.


\noindent \textbf{RevA, Comment-2.} \texttt{``However in all of these results the critical variable seems to be that there is a gap between what the attacker and defender know. Perhaps the idea is that for synthetic text in the wild, the defense will not know exactly how the generation model works. But this point is not discussed in depth and I feel that discussing it would strengthen the paper. Indeed, I suspect that if the defense is optimally fine-tuned to the synthetic text generation procedure (i.e., fine-tuned on it, knows the exact decoding strategy, etc.) then the performance of the detectors may be as good as advertised.''} 

\textit{Response:} We have addressed this concern. Please see the response to Major-Rev, Comment-10 in Section~\ref{sec:mjrev}.
% We will better discuss this point in the earlier sections. 
% Under a realistic detection scenario, the defender has limited or no a priori knowledge about synthetic text generation procedure in the wild. For example, when collecting data from text-generation services, no more information was provided for us except that transformer-family LMs are used. Our goals (stated in section II.B) focus on understanding and improving performance in the wild, and also understanding performance against adaptive attackers. Our results (see comment \#1) does indicate that fine-tuning the defense towards a specific attack is a way forward. But the defender may have to frequently adapt their defenses against new attacker strategies.

\noindent \textbf{RevA, Comment-3.} \texttt{``... I do think that the paper makes a compelling case that simply using off-the-shelf detectors on synthetic text in the wild does not work. This is not too surprising simply because the distribution of synthetic text in the wild is likely different than that of the training data of the detectors. Nevertheless, settling this question experimentally makes sense. Similarly, the finding that an adaptive attacker that simply changes the decoding strategy or that uses conditional text for generation is not too surprising in hindsight because again it changes the distribution of synthetic text compared to what the defense expects''}

\textit{Response:} We are glad to see that the reviewer sees value in experimentally validating this question. That said, even though our research questions may appear simple, our findings provide concrete actionable insights for future work: (1) Prior work showed that using hand-crafted features are sufficient for synthetic text detection (GLTR), or that fine-tuned Transformer models learning complex features (GROVER) work extremely well in detecting synthetic text. We find that both such approaches suffer significantly against simple (low-cost) evasion strategies, \eg by simply changing the decoding strategy. The attacker does not need to re-train the text generator on a new dataset to evade detection. (2) Instead, focusing more on defenses leveraging semantic features (FAST) would be a more promising approach, moving forward. 

\noindent \textbf{RevA, Comment-4.} \texttt{``...there is no experiment to study whether length of documents matter in detection. I understand that some defenses require a minimum document length, but document length seems like an important variable that should be accounted for. (It also appears that in the initial experiments, there is a significant length difference between synthetic documents and real documents.)''}

 \textit{Response:} We have addressed this concern. Please read our response to Major-Rev, Comment-9 in Section~\ref{sec:mjrev}.
%  We want to clarify that lengths of real and synthetic documents used in detection are the same. While the length of the documents in the synthetic and real class as well as across different datasets may be different,  detection is only based on the length of the article within the classifier’s context window. Hence length differences do not impact any of our findings.
 
%   To fully address reviewer's concern, we made the following changes: (1) We use a predefined uniform context window size for each defense, \eg each defense can use a maximum of 512 tokens. This impacts 3 defenses, \ie \gbert{}, \grover{}, and \gltrgpt{}, which previously used different context window sizes. To make the change, we updated all the experiments associated with these 3 defenses. Such a change does not change any of our major findings. 
%   (2) We added experiments studying the impact of varying the context window size, \ie 64, 128, 256, 512 tokens. We observe a linear trend for all defenses that the evaluation performance monotonically improves as the context window size under detection increases, shown in Figure~\ref{fig:baseline_token_length}.


\noindent \textbf{RevA, Comment-5.} \texttt{``Another example is that it is unclear how similar the real and synthetic documents really are. I understand that it is difficult to have a metric to measure the distance between the two distributions, but without some idea of this it is difficult to interpret the results. Ideally one would have some idea of the distribution shift between the training set of the detector and the In-the-wild set so that the percentage change in F1-score $\Delta F1$ can be interpreted relative to it. In fact, I am not convinced that F1-score of the synthetic class or recall of the synthetic class are meaningful metrics here. Why not use AUC?''}

\textit{Response:} 
%We focus on three aspects to address the reviewer's concerns: 
(1) We took care to ensure that the synthetic and real articles are connected in some way. 
We followed the methodology from prior work to generate synthetic articles. For example, when generating In-the-wild datasets, we used the article title from a real document as context to generate a corresponding synthetic article. For evaluating GROVER, RoBERTA-Defense, FAST, and DistilFAST, we used the real data's context to generate synthetic data, \ie title, date, website name. For evaluating GLTR and BERT-Defense, the synthetic data and real data are similar at a high level because the real data was used to train the models which we used to generate the synthetic articles from.

(2) We have addressed the concern about measuring the distribution shift between the training set of the detector and the In-the-wild set. Please read our response to Major-Rev, Comment-4 in Section~\ref{sec:mjrev}.

(3) We added AUC ROC as a complementary metric for detection performance in Table~\ref{tab:defenses-setup}. We found that different prior works use different metrics, with one work using some “unrealistic” metrics as well (paired accuracy in GROVER, see Section~\ref{sec:six_defenses_info}). For our study, it is important to have a single consistent metric for all our evaluation, that is also easy to interpret. A metric like F1 provides insights into detection performance, and does not delegate the task of calibrating a decision threshold to future work. In practice, one would be expected to draw a threshold on the prediction score. In that regard, F1 presents an easier to interpret detection performance metric compared to AUC. Also, Precision and Recall also provide insights into the false positive and false negative rate.


\subsection{Response to Review B}
\label{sec:revb}
% \subsubsection{Detailed Review Comments}

\noindent \textbf{RevB, Comment-1.} \texttt{``Overall, this is an interesting and timely study. No major problem with the evaluation.''}

\textit{Response: } We thank the reviewer for the positive feedback.

\noindent \textbf{RevB, Comment-2.} \texttt{``Quality of writing.''}

\textit{Response: } We have addressed this concern. Please see the response to Major-Rev, Comment-2 in Section~\ref{sec:mjrev}.

\noindent \textbf{RevB, Comment-3.} \texttt{``Some details missing.''}

\textit{Response: } To address this concern, we make sure all the important details of experiments are covered in the revision draft. We addressed all the concerns raised by reviewers. We provided more technical details of our \ourattack{} pipeline. In the Appendix section, we added more details of our experimental settings and metric choices. 

For more details about how we improve the paper, you may also read the responses to Major-Rev, Comment-2 and Major-Rev, Comment-4 in Section~\ref{sec:mjrev}.


\noindent \textbf{RevB, Comment-4.} \texttt{``Too much text; tables sometimes hard to read/parse.''}

\textit{Response:} To address this concern, we made our text as concise as possible, and improved all the tables and captions.

\subsection{Response to Review C}
\label{sec:revc}
% \subsubsection{Detailed Review Comments}
\noindent \textbf{RevC, Comment-1.} \texttt{``The background section presents readers with good preliminary information about the approach, but it can be extended to include more concepts such as the Temperature decoding approach.''}

\textit{Response: } 
To address this concern, we discuss the Temperature decoding approach under \textit{``Text decoding strategies''} of Section~\ref{sec:background}.

%\jiameng{synced with main body text}
We replicate the discussion here:
Temperature sampling~\cite{ackley1985learning}, shapes the probability distribution by dividing the logits by a temperature parameter before passing them to the softmax function.
Low temperatures make the model produce less diverse text, as it makes more confident predictions (tokens), while temperatures greater than 1, result in more diverse text, as confidence is decreased.
%The simplest decoding strategy is greedy sampling, where the most probable next token is chosen. However, temperature sampling and greedy sampling tend to produce repetitive text~\cite{holtzman2019curious}.

%Specifically, Temperature sampling~\cite{ackley1985learning}, shapes the probability distribution by dividing the logits by a temperature parameter before passing them to the softmax function.
%Low temperatures make the model produce less diverse text, as it makes more confident predictions (tokens), while temperatures greater than 1, result in more diverse text, as confidence is decreased.

\noindent \textbf{RevC, Comment-2.} \texttt{``While fine-tuning the models, Table IV. The authors did not consider GLTR defense and mentioned that the GLTR’s classifier is not DNN-based. Also, the authors stated that since the code for logistic regression was not released by the original authors they have re-implemented it, probably, using scikit-learn ML library. Why did the authors not re-implement the logistic regression using the TensorFlow framework, from the ground up, to make it possible for fine-tuning? Have the authors ever considered this?''}

\textit{Response: } 
We have addressed these concerns. Please read our responses to Major-Rev, Comment-5 and Major-Rev, Comment-6 in Section~\ref{sec:mjrev}.

%We have addressed the concerns by including GLTR defense in fine-tuning experiments. Please read the responses to Major-Rev, Comment-5 and Major-Rev, Comment-6 in Section~\ref{sec:mjrev}.
% Fine-tuning as a method for domain adaptation or transfer learning is designed for DNN-based language models~\footnote{\url{https://ruder.io/recent-advances-lm-fine-tuning/}}. GLTR does not use a DNN model for classification. Implementing it in TensorFlow does not change the underlying model. Hence, we did not consider it in the fine-tuning experiments. 

% We have addressed the concern by making the following changes: (1) We reconsidered the GLTR defenses for the fine-tuning experiments, and conducted a new set of experiments for the GLTR defenses. (2) We re-implemented the logistic regression classification to make sure that all the parameters were carefully tuned. For details of both changes, please read responses to Quote 6 and Quote 7 in Section~\ref{sec:mjrev}. 


\noindent \textbf{RevC, Comment-3.} \texttt{``The authors reported a better F1 score for BERT-Defense in their setup compared to the original work. They mentioned this is likely because of selecting a smaller batch size while training the algorithm. This statement may not be held since the original dataset used for training the BERT-Defense was not available to the authors. To have a fair comparison both datasets should be identical.''}

\textit{Response: } 
We understand the reviewer's concern and agree with the reviewer's opinion. The reviewer is correct that the datasets used to train BERT-Defense in the original work and in our work are not identical, but similar. The real data for both the classifiers came from the same publicly released WebText dataset and the synthetic data was generated using the same model, and decoding strategy as well as conditional text generation process. 

To address the concern, we removed the statement that change in batch size likely resulted in the performance difference. Furthermore, in this revision, we had to retrain the \gbert{} model. To allow fair comparison among defenses, we changed the context window size of \gbert{} for detection from 192 tokens to 512 tokens, thus retrained a new \gbert{}. With the new \gbert{} setup, we achieved a higher F1 score than the original model, even after using a smaller training set (10,000 articles per class Vs 250,000 articles in the original work). Our model uses the full context window size of 512 tokens, supported by BERT, unlike the smaller window size of 192 tokens in the original work. We suspect the higher performance is likely due to the larger context window used by our implementation. 

 %Instead, (1) we clearly explained how we set up \gbert{} (See Table~\ref{tab:defenses-setup} for details). (2) We suggest ``the higher performance is likely due to the larger context window used by our implementation.'' \jiameng{not sure if the review will be happy about our assumption again.} 



\noindent \textbf{RevC, Comment-4.} \texttt{``For instance, the datasets of BERT-Defense and RoBERTa-Defense differ. As it can be seen from Table I, BERT-Defense does a better job detecting deepfake text compared to RoBERTa-Defense. On the other hand, as clearly stated in the paper, RoBERTa-Defense makes several improvements to the BERT and is known to outperform BERT in NLP tasks. How can the authors justify this?''}

\textit{Response:} 
We understand the reviewer's concern. We justify our statement in two aspects: (1) The baseline performances of \gbert{} and \rbert{} are not actually comparable. For the baseline results in Table~\ref{tab:defenses-setup}, we aimed to replicate the defense results in their original setup. Therefore, in Table~\ref{tab:defenses-setup}, the datasets used to test RoBERTa-Defense and BERT-Defense are different and this means we cannot simply compare the baseline performances of both to conclude which one is better. The synthetic text for testing BERT-Defense was generated from GPT2-L which is a model that is around half the size of the GROVER-Mega model used to test RoBERTa-Defense. Smaller models generally end up leaving more statistical artifacts in generated text which classifiers can accurately detect. This probably explains the higher performance of BERT-Defense when compared to RoBERTa-Defense in Table~\ref{tab:defenses-setup}. (2) Instead, if we look at the performance of BERT-Defense and RoBERTa-Defense on our In-the-wild datasets in Table~\ref{tab:eval_in_the_wild}, we can clearly observe the superior performance of RoBERTa-Defense.



% %(2) \rbert{} did perform better on detecting In-the-wild synthetic documents than \gbert{} does.

% Here is our detailed explanation: (1)   

\noindent \textbf{RevC, Comment-5.} \texttt{``In Table I, although the BERT-Defense and GLTR share the same ML backend and only differ in the last layer classifier, there is a significant change in the reported F1 score, given the same dataset. I was wondering if hyperparameters of the logistic regression classifier were carefully tuned.''}

\textit{Response:} 
(1) We want to clarify that BERT-Defense and GLTR (using BERT as a backend) are very different defense schemes and we believe that is the reason behind the difference in their performance. As explained in Section~\ref{sec:six_defenses_info}, GLTR uses hand-crafted features, \ie binned token probabilities that are extracted using a backend language model and then uses a logistic classifier to discriminate between real and fake text. On the other hand, BERT-defense takes full advantage of the BERT model to extract complex sequential features from the articles. Moreover, the entire BERT-model is fine-tuned for BERT-defense as opposed to training just the logistic classifier in GLTR.
(2) In this revision, we re-implemented the logistic regression classifier with grid search to ensure hyperparameters are properly tuned. Please read our response to Major-Rev, Comment-6 in Section~\ref{sec:mjrev} for more details.
% Please read the response to Major-Rev, Comment-6 in Section~\ref{sec:mjrev}.

% Here is our detailed explanation: (1) We want to clarify that BERT-Defense and GLTR using BERT as a backend are very different defense schemes and we believe that is the reason behind the difference in their performance. As explained in Section~\ref{sec:six_defenses_info}, GLTR uses hand-crafted features, \ie binned token probabilities that are extracted using a backend language model and then uses a logistic classifier to discriminate between real and fake text. On the other hand, BERT-defense takes full advantage of the BERT model to extract complex sequential features from the articles. Moreover, the entire BERT-model is fine-tuned for BERT-defense as opposed to training just the logistic classifier in GLTR. (2) 
% % We confirmed the GLTR configuration with the authors of the GLTR paper, and they recommended using the default parameter settings in scikit-learn for logistic regression to implement GLTR. 
% To address reviewer's concern, we applied grid search on a set of hyperparameters while training the logistic regression classifier to assure the classifier are carefully tuned. Please read the response to Major-Rev, Comment-6 in Section~\ref{sec:mjrev} for more details.

% \textit{Response:} 
% We understand the reviewer's concern and respond in the following two aspects: (1) BERT-Defense and GLTR (using BERT as a backend) are very different defense schemes. (2) In this revision, we re-implemented the logistic regression classifier with grid search to ensure hyperparameters are properly tuned. 
% % Please read the response to Major-Rev, Comment-6 in Section~\ref{sec:mjrev}.

% Here is our detailed explanation: (1) We want to clarify that BERT-Defense and GLTR using BERT as a backend are very different defense schemes and we believe that is the reason behind the difference in their performance. As explained in Section~\ref{sec:six_defenses_info}, GLTR uses hand-crafted features, \ie binned token probabilities that are extracted using a backend language model and then uses a logistic classifier to discriminate between real and fake text. On the other hand, BERT-defense takes full advantage of the BERT model to extract complex sequential features from the articles. Moreover, the entire BERT-model is fine-tuned for BERT-defense as opposed to training just the logistic classifier in GLTR. (2) 
% % We confirmed the GLTR configuration with the authors of the GLTR paper, and they recommended using the default parameter settings in scikit-learn for logistic regression to implement GLTR. 
% To address reviewer's concern, we applied grid search on a set of hyperparameters while training the logistic regression classifier to assure the classifier are carefully tuned. Please read the response to Major-Rev, Comment-6 in Section~\ref{sec:mjrev} for more details.



\noindent \textbf{RevC, Comment-6.} \texttt{``In finding 2, the authors stated that bidirectional models, if robustly trained, perform better than unidirectional models. But according to Table IV, after fine-tuning the GROVER (unidirectional model) outperforms BERT-Defense (Bidirectional model). How can the authors explain this?''}

\textit{Response: } 
We have addressed this concern. Please see our response to Major-Rev, Comment-7 in Section~\ref{sec:mjrev}.
% The reviewer is concerned about the finding ``\textit{Robustly pre-trained bidirectional models generalize better than unidirectional models}'' (It is Finding 2 in the current draft). ``Table IV'' mentioned in the quote is Table~\ref{tab:fine_tune_wild} in the current draft.

% (1) There seems to be some confusion about which model we were referring to in this finding. To quote from the paper, we wrote, “Robustly pre-trained bidirectional models generalize better than unidirectional models” and this was referring to the RoBERTa-Defense. ‘Robustly pre-trained’ was a reference to the meaning of RoBERTA which is “Robustly optimized BERT”. We stated this finding because we observed that the RoBERTa-Defense actually performed better on the In-the-wild datasets than it did on the baseline test dataset. (2) This finding is not related to the fine-tuning experiments in Table~\ref{tab:fine_tune_wild} which shows results for BERT-Defense, and not RoBERTa. 
% To address this concern, we modified our statement of the finding as ``Robustly pre-trained bidirectional models, \ie RoBERTa, generalize better than unidirectional models.'' to avoid the confusion. 


\noindent \textbf{RevC, Comment-7.} \texttt{``The authors, in table III, have reported some results and mentioned that they are unable to explain them. Now, my question is, why do the authors in a scientific work bring such results that cannot talk about them!''}

\textit{Response: }This is regarding the performance disparity between \gltrgpt{} and \gltrbert{} on the In-the-wild datasets (in Table~\ref{tab:eval_in_the_wild}). We removed the statement saying that we do not understand this result, and now provide an explanation in Section~\ref{sec:detection_performance_defenses}. \gltrgpt{} and \gltrbert{} are trained and tested on the same datasets. The only difference between the two defenses is the backend LM used to craft features for discrimination. Therefore, we believe the performance disparity is caused by how the backend model infers input text samples. In other words, the back-end LM model (BERT vs GPT-2) used by GLTR can have a huge impact on generalization performance.


That said, DNN-based inference is inherently hard to explain and interpreting how DNNs make decisions is a field into itself and it is beyond the scope of this paper to dive deeply into explaining DNN-based predictions. As explained in the paper “Intriguing properties of neural networks” by Szegedy et al, DNNs often learn solutions that are uninterpretable and possess counter-intuitive properties.

%We were not able to explain this result in our previous submission, so we highlighted the need to leverage explainable AI systems to understand the failures and successes of DNN-based synthetic text detection schemes. 


% (1) \gltrgpt{} and \gltrbert{} are trained and tested on the same datasets. The only difference between them is the backend model used to craft features for discrimination.
% Therefore, we believe the performance disparity is caused by how the backend model infers input text samples. That said, DNN-based inference is inherently hard to explain and interpreting how DNNs make decisions is a field into itself and it is beyond the scope of this paper to dive deeply into explaining DNN-based predictions. As explained in the paper~\cite{szegedy2013intriguing} by Szegedy \etal{}, DNNs often learn solutions that are uninterpretable and possess counter-intuitive properties. 
% (2) We understand the reviewer's concern. In this revision, we removed previous statement and instead emphasized the fact that the back-end LM model (BERT vs GPT-2) used by GLTR can have a huge impact on generalization performance. 



% DNN-based inference is inherently hard to explain and interpreting how DNNs make decisions is a field into itself and it is beyond the scope of this paper to dive deeply into explaining DNN-based predictions. As explained in the paper “Intriguing properties of neural networks” by Szegedy et al, DNNs often learn solutions that are uninterpretable and possess counter-intuitive properties.

% We understand the reviewer's concern. 
% This is regarding the performance disparity between \gltrgpt{} and \gltrbert{} on In-the-wild datasets (in Table~\ref{tab:eval_in_the_wild}). We were not able to explain this result in our previous submission, so we highlighted the need to leverage explainable AI systems to understand the failures and successes of DNN-based synthetic text detection schemes. 


% (1) \gltrgpt{} and \gltrbert{} are trained and tested on the same datasets. The only difference between them is the backend model used to craft features for discrimination.
% Therefore, we believe the performance disparity is caused by how the backend model infers input text samples. That said, DNN-based inference is inherently hard to explain and interpreting how DNNs make decisions is a field into itself and it is beyond the scope of this paper to dive deeply into explaining DNN-based predictions. As explained in the paper~\cite{szegedy2013intriguing} by Szegedy \etal{}, DNNs often learn solutions that are uninterpretable and possess counter-intuitive properties. 
% (2) We understand the reviewer's concern. In this revision, we removed previous statement and instead emphasized the fact that the back-end LM model (BERT vs GPT-2) used by GLTR can have a huge impact on generalization performance. 

% Furthermore, in Section~\ref{sec:discussion} of the paper, we highlight the need to leverage explainable AI systems to understand the failures and successes of DNN-based synthetic text detection schemes. 


\noindent \textbf{RevC, Comment-8.} \texttt{``I also would like to see an analysis of the number of tokens used for perturbations. Currently, this number is set to 10 tokens. I was wondering how this can influence the evasion rate.''}

\textit{Response: } We have addressed this concern. Please see our response to Major-Rev, Comment-8 in Section~\ref{sec:mjrev}.
% To address this concern, we made the following change: (1) We experimented with different numbers of total perturbations made to the text. We experimented with 5, 10, 15 and 20 tokens perturbed in total.  We observe that, while the Evasion Rate (ER) was higher with more perturbations, the text quality, as indicated by the GRUEN metric, tends to degrade. Therefore, it is a trade-off between Evasion Rate and preserving the text quality.

\noindent \textbf{RevC, Comment-9.} \texttt{``Last but not the least, do the authors intend to share their In-the-wild synthetic dataset with the research community?''}

\textit{Response: } As we mentioned at the end of the introduction section, we will release our synthetic datasets to the research community. 

\noindent \textbf{RevC, Comment-10.} \texttt{``Lack of sufficient technical details regarding process of adversarial examples generation''}

\textit{Response:} We have addressed this concern. Please see our response to Major-Rev, Comment-4 in Section~\ref{sec:mjrev}.
% We currently provide details of DFTFooler in Section V-A, page 9. We will further add any details required to completely reproduce our results. We will also release code implementing our new adversarial attack scheme.


\noindent \textbf{RevC, Comment-11.} \texttt{``... adding adversarial perturbations to existing synthetic text samples … has mediocre novelty given other similar lines of works. The idea of replacing words in a sentence with words that are close in its embedding space which causes a change in the predicted class is not novel [R1].''}

\textit{Response: } 
We want to clarify that \textit{novelty is not in finding words close in an embedding space, but instead in finding which words to replace, and to find the right placement word among the many possible replacement options.} Existing work such as TextFooler identifies important words to replace by either querying the victim model a large number of times or by querying a local classifier that is an approximation of the victim classifier. Our approach, DFTFooler, is novel because it does not require both these features --- \ie does not require any queries to the victim classifier, nor a shadow classification model. DFTFooler leverages properties that are unique to the synthetic text detection space to identify important words to replace. To achieve this, we only require widely available pre-trained language models (\eg BERT, GPT-2) to identify perturbations that would flip the decision. Our work further highlights how pre-trained language models can be misused to craft adversarial inputs. We added more details of our \ourattack{} attack in Section~\ref{sec:dftfooler_tech_details}.


% \textcolor{blue}{To address this concern, we added a discussion regarding the novelty of \ourattack{} compared to existing adversarial attacks in Section~\ref{sec:adaptive-attack-methods}.} \jiameng{did you add it?}
% We thank reviewer's comment on this. We want to clarify that \textit{Novelty is not in finding words close in an embedding space, but instead in finding which words to replace.} Existing work such as TextFooler identifies important words to replace by either querying the victim model a large number of times or by querying a local classifier that is an approximation of the victim classifier. Our approach, DFTFooler, is novel because it does not require both these features --- \ie does not require any queries to the victim classifier, nor a shadow classification model. DFTFooler leverages properties that are unique to the synthetic text detection space to identify important words to replace. To achieve this, we only require widely available pre-trained language models (\eg BERT, GPT-2) to identify perturbations that would flip the decision. Our work further highlights how pre-trained language models can be weaponized to craft adversarial inputs. 


\subsection{Response to Review D}
\label{sec:revd}
% \subsubsection{Detailed Review Comments}

\noindent \textbf{RevD, Comment-1.} \texttt{``The robustness of deepfake detectors has been studied in image domain [A, B, C]. … The discussion on the similarity/difference between deepfake image/text detection would be appreciated.''}

\textit{Response: } Thanks for the pointers. We have addressed this concern. Please see our response to Major-Rev, Comment-1 in Section~\ref{sec:mjrev}.


\noindent \textbf{RevD, Comment-2.} \texttt{``Some claims seem not convincing. Please clarify. For instance, when comparing the adversarial examples, the authors claimed that “DFTFooler also outperforms the random perturbation scheme for all defenses.” This does not match the results shown in Table VII. In Table VII, DFTFooler with BERT backend achieves marginally higher ER than random perturbation. However, its GRN-AFTER is lower than random perturbation. This may not mean DFTFooler is better considering the trade-off. Moreover, DFTFooler with GPT2-XL backend even has lower ER than random perturbation.''}

\textit{Response: } 
We have addressed this concern. Please see our response to Major-Rev, Comment-7 in Section~\ref{sec:mjrev}.
% The reviewer is concerned about the explanation of the finding ``\textit{\ourattack{} can generate transferable adversarial samples}'' (It is Finding 7 in the current draft).
% To address this concern, we clarified the explanation of this part under Finding 7 in Section~\ref{sec:adaptive-attack-eval}. 

% A major change in this revision work is that we make the context window size of each defense uniform in size \ie we use the first 512 tokens of an input document. (We made this change due to the Major-Rev, Comment-8 in Section~\ref{sec:mjrev}). Since adversarial attacks are suppose to perturb words within the context window, we need to rerun all the adversarial attack experiments for \gbert{}, \gltrgpt{}, and \grover{}, of which the context window size has been changed. Therefore,
% We rerun all the adversarial attack experiments for the above defenses and updated all the results in Table~\ref{tab:adversarial_perturbs_results}.

% With the updated evalaution results, we need to clarify 2 points: \textit{(1) Despite what the reviewer observed in our previous submission, after we rerun the experiments, we observe that DFTFooler with both BERT and GPT-2 backend outperform the random perturbation attack for all the defenses.} 
% Specifically, DFTFooler with BERT backend show significant percentage increase in ER (Evasion Rate) ranging from 35.8\% to 95.0\% compared to random perturbation,
% while DFTFooler with GPT2-XL backend show percentage increase in ER ranging from 18.8\% to 73.5\% compared to random perturbation. 
% (2) Note that, unlike TextFooler, DFTFooler achieves such attack performance rates without a single query to the victim classifier, which is a more challenging attack. \textcolor{blue}{Figure~\ref{fig:ROBERTA_CDF_5curves_response} below shows how close the GRUEN score distributions are for DFTFooler, TextFooler and random perturbation attack.} 


\noindent \textbf{RevD, Comment-3.} \texttt{``Some explanations for some findings are unhelpful. For instance, `Defenses trained on conditionally generated text are not able to detect unconditionally generated text.' Is there any explanation why this happens?''}

\textit{Response: } 
We have addressed this concern. Please see our response to Major-Rev, Comment-7 in Section~\ref{sec:mjrev}.
% The reviewer is concerned about the explanation of the finding ``\textit{Defenses trained on conditionally generated text are not able to detect unconditionally generated text}'' (It is Finding 6 in the current draft).
% To address the concern, we provided a detailed explanation under Finding 6 in Section~\ref{sec:adaptive-attack-eval}. 

% This is our explanation: We believe that this is because defenses trained on conditionally generated text learn a narrow distribution of synthetic text because language models are conditional probability models and an initial priming token can alter the distribution of the generated text. We can think of LMs as being in a particular state space at each time-step. If the priming tokens lead the model into a particular state space which the model might not have reached on it’s own due to those ‘priming tokens’ being low probability tokens, and thus less likely to be sampled in an unconditional setting, then conditionally trained models might learn a narrower distribution of synthetically generated text and not generalize well to unconditionally generated text. 

\noindent \textbf{RevD, Comment-4.} \texttt{``It is better to have some explanation in table captions about what ‘--’ represents and why.''}

\textit{Response: } To address this concern, we updated the table captions to explain all the ‘--’. 

‘--’ represents experiments we ignored due to different reasons: 
(1) ‘--’ in Table~\ref{tab:eval_in_the_wild} and ~\ref{tab:fine_tune_wild}: We did not test GROVER, FAST and RoBERTa-Defense on non-news domain datasets, which includes Kafkai and RedditBot. This is because these defenses are only trained for the news domain. 
% Exactly the same reason for ‘--’ in Table~\ref{tab:fine_tune_wild}. 
(2) ‘--’ in Table~\ref{tab:decoding_eval_short}: For Temperature decoding, we only show results for GLTR defenses, because the original GLTR work was evaluated using temperature based decoding. Temperature decoding is known to produce repetitive and low quality text compared to other decoding strategies, so we omit this for the other defenses.
% (3) `--' in Table~\ref{tab:distribution_shift} means not-applicable observations. `D-B' does not apply to \textit{in-the-wild} datasets, `D-W' does not apply to the baseline dataset. Plus, \grover{} was not evaluated against Kafkai and GPT-3 Reddit bot datasets.
(3) ‘--’ in Table~\ref{tab:adversarial_perturbs_results}: At the time, we were unable to implement the TextFooler attack against GLTR, GROVER and FAST due to various challenges. However, we have solved these challenges and now have the missing results. 


